A conditional gradient homotopy method with applications to Semidefinite Programming

We propose a new homotopy-based conditional gradient method for solving convex optimization problems with a large number of simple conic constraints. Instances of this template naturally appear in semidefinite programming problems arising as convex relaxations of combinatorial optimization problems. Our method is a double-loop algorithm in which the conic constraint is treated via a self-concordant barrier, and the inner loop employs a conditional gradient algorithm to approximate the analytic central path, while the outer loop updates the accuracy imposed on the temporal solution and the homotopy parameter. Our theoretical iteration complexity is competitive when confronted to state-of-the-art SDP solvers, with the decisive advantage of cheap projection-free subroutines. Preliminary numerical experiments are provided for illustrating the practical performance of the method.

==> LineSearch.tex <==
%%----------------------------------------------------------------------
%%% Line search
%----------------------------------------------------------------------
% !TEX root = ./FW_SDP.tex
%

\subsection{Line Search}
The step size policy employed in Algorithm \ref{alg:CndG} is inversely proportional to the local norm $\ce_{t}(x)$. In particular, its derivation is based on the a-priori restriction that we force our iterates to stay within a trust-region defined by the Dikin ellipsoid. This restriction may force the method to take very small steps, and as a result display bad performance in practice. A simple remedy to this is to employ a line search strategy. Given $(x,t)\in\dom(F)\times(0,+\infty)$, let 
\begin{equation}\label{eq:ExactLS}
\gamma_{t}(x)=\argmin_{\gamma\in[0,1]\text{ s.t. } x+\gamma(s_{t}(x)-x) \in \dom(F)}V_{t}(x+\gamma(s_{t}(x)-x)).
\end{equation}
%=== CnDG - Line Search==========
\begin{algorithm}[t]
 \caption{\ac{CndG} with line search: $\LCG(x^{0},\eps,t)$}
 \label{alg:LineSearchCndG}
 \begin{algorithmic}
\State {\bfseries Input: } $(x^{0},t)\in\setC\times(0,\infty)$ initial state; $\eps>0$ accuracy level
%\REPEAT 
\For{$k=0,1,\ldots$}
 \If{$\gap_{t}(x^{k})>\eps$}
\State Same as Algorithm \ref{alg:CndG}, but with step size strategy \eqref{eq:ExactLS}.
\Else
  \State \ms{STOP. Return $k$ and $x^{k}$.}
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
%============================
Thanks to the barrier structure of the potential function $V_{t}$, some useful consequences can be drawn from the definition of $\gamma_{t}(x)$. First, $\gamma_{t}(x)\in\{\gamma\geq 0\vert x+\gamma(s_{t}(x)-x)\in\dom(F)\}$. This implies $x+\gamma_{t}(x)(s_{t}(x)-x)\in\setX\cap\dom(F)\cap\dom(g)$. Second, since $\alpha_{t}(x)$ is also contained in the latter set, we have 
\[
V_{t}(x+\gamma_{t}(x)(s_{t}(x)-x))\leq V_{t}(x+\alpha_{t}(x)(s_{t}(x)-x))\qquad\forall (x,t)\in\dom(F)\times(0,+\infty).
\]
Via a comparison principle, this allows us to deduce the analysis of the sequence produced by $\LCG(x^{0},\eps,t)$ from the analysis of the sequence induced by $\CG(x^{0},\eps,t)$.
Indeed, if $\{\xi^{k}_{t}\}_{k \geq 0}$ is the sequence constructed by the line search procedure $\LCG(x^{0},\eta,t)$, then we have 
$V_{t}(\xi^{k+1}_{t})\leq V_{t}(\xi_{t}^{k}+\alpha_{t}(\xi^{k}_{t})(s_{t}(\xi^{k}_{t})-x^{k}_{t}))$ for all $k$. 
Hence, we can perform the complexity analysis on the majorizing function as in the analysis of procedure $\CG(x^{0},\eps,t)$. 
Consequently, all the complexity-related estimates for the method $\CG(x^{0},\eta,t)$ apply verbatim to the sequence $\{\xi^{k}_{t}\}_{k\geq 0}$ induced by the method $\LCG(x^{0},\eta,t)$. 

%%%%Inexact LMO%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
\subsection{Inexact Implementation}
Algorithm \ref{alg:CndG} assumes that the \ac{LMO} performs exact computation of the search direction $s_t(x)$. This may not be directly available in practice. Just like in \cite{Jag13}, we show that our analysis carries essentially through even in the relaxed \ac{LMO} model with inexact implementation. Let $\gamma\in[0,1)$ be a given parameter, measuring the approximation quality of the oracle \eqref{eq:LMO} relative to the target accuracy $\eta$. Instead of the search direction $s_{t}(x)$, suppose the \ac{LMO} returns us a point $\tilde{s}_t=\tilde{s}_{t}(x)$ satisfying 
\begin{equation}\label{eq:inexact}
t^{-1}F'(x)[\tilde{s}_{t}(x)]+g(\tilde{s}_{t}(x))\leq\min_{s\in\setX}\left\{t^{-1}F'(x)[s]+g(s)\right\}+\gamma\eta.
\end{equation}
Following the derivations performed in the exact computational model, we are defining the inexact gap function 
\begin{equation}
\widetilde{\gap}_{t}(x):=t^{-1}F'(x)[x-\tilde{s}_{t}(x)]+g(x)-g(\tilde{s}_{t}(x)),
\end{equation}
and the associated analytic step size policy, using  $\tilde{\ce}_{t}(x):=\norm{\tilde{s}_{t}(x)-x}_{x}$, 
\begin{equation}\label{eq:inexactstep}
\tilde{\alpha}_{t}(x)=\min\left\{1,\frac{t\widetilde{\gap}_{t}(x)}{\tilde{\ce}_{t}(x)(\tilde{\ce}_{t}(x)+t\widetilde{\gap}_{t}(x))}\right\}.
\end{equation}
%where $\tilde{e}_{t}(x):=\norm{\tilde{s}_{t}(x)-x}_{x}$. 
%=== CnDG - Approximate linear subproblems==========
\begin{algorithm}[t]
 \caption{\ac{CndG} with inexact oracle: $\ICG(x^{0},\eps,t)$}
 \label{alg:ApproxCG}
 \begin{algorithmic}
\State {\bfseries Input: } $(x^{0},t)\in\setC\times(0,\infty)$ initial state; $\eps>0$ accuracy level, $\gamma\in[0,1)$ inexactness parameter
%\REPEAT 
\For{$k=0,1,\ldots$}
 \If{$\widetilde{\gap}_{t}(x)>(1-\gamma)\eps$}
\State Find $\tilde{s}^{k}= \tilde{s}_{t}(x^{k})\in\setX$ such that \eqref{eq:inexact} holds at $x^{k}$.
\State Set $\alpha_{k}=\tilde{\alpha}_{t}(x^{k})$ by evaluating eq. \eqref{eq:inexactstep}.
\State Update $x^{k+1}=x^{k}+\alpha_{k}(\tilde{s}^{k}-x^{k})$. 
 \Else
  \State Return $x^{k}$.
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
%============================
\begin{remark}
Note that as $\eta\to0$, the \ac{LMO}'s accuracy as defined in \eqref{eq:inexact} improves. \cite{Jag13} achieves such an improving oracle by coupling the accuracy imposed on the subproblem solver with the $1/k$-step size policy employed in the vanilla \ac{CndG}.  
\end{remark}
The next propositions are the resulting iteration complexity statements of Algorithm $\ICG(x^{0},\eta,t)$, mimicking the statements in Proposition \ref{prop:Delta} and \ref{prop:gap}. Since the analysis of the inexact implementation regime is analogous to the exact \ac{LMO} model, we provide sketches of proofs of these statements in Section \ref{sec:inexactanalysis}. 
%%%%%%%%%%
\begin{proposition}\label{prop:Delta-Inexact}
Algorithm $\ICG(x^{0}_{t},\eta,t)$ requries at most $\tilde{N}_{\gamma}(x^{0}_{t},\eta,t)$ iterations, in order to reach a point satisfying $\Delta_{t}(x^{k}_{t})\leq \eta$, where
\begin{equation}
\tilde{N}_{\gamma}(x^{0}_{t},\eta,t):=K_{t,\gamma}(x^{0}_{t})+\lceil 12(\nu+t\Omega_{g})^{2}\left(\frac{1}{t\eta}-\frac{1}{t(\Delta_{t}(x^{0}_{t})-\gamma\eta)}\right)^{+}\rceil,
\end{equation}
and 
\begin{equation}\label{eq:K}
K_{t,\gamma}(x^{0}_{t}):=\left\{\begin{array}{ll}
0 & \text{ if }\gamma\eta \geq\frac{1}{10.6t}\\ 
\lceil 5.3(\nu+t(\Omega_{g}-\gamma\eta)+t\Delta_{t}(x^{0}_{t}))\rceil \log\left(\frac{10.6t\Delta_{t}(x^{0}_{t})}{1-10.6t\gamma\eta}\right) & \text{if }\gamma\eta<\frac{1}{10.6t}.
\end{array}\right.
\end{equation}
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop:gap-Inexact}
Given $\eta,t>0$ and $\gamma\in(0,1/3)$. Let $\tilde{R}(x^{0}_{t},\eta,t)$ be the first iterate $k$ satisfying $\gap_{t}(x^{k}_{t})\leq\eta$ for Algorithm $\ICG(x^{0},\eta,t)$. Then 
$$
\tilde{R}_{\gamma}(x^{0}_{t},\eta,t)\leq K_{t,\gamma}(x^{0}_{t})+\lceil \frac{24}{t(1-\gamma)\eta}(\nu+t\Omega_{g})^{2}\rceil,
$$
where $K_{t,\gamma}(x^{0}_{t})$ is defined in \eqref{eq:K}. 
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}
Observe that all the complexity estimates reduce to the ones proved for the exact oracle model by setting $\gamma=0$.
\end{remark}
Based on the above estimates, it becomes clear that the worst-case bounds on the overall iteration complexity of $\texttt{Homotopy}(x^{0},\eps,f)$ with $\ICG(x^{0},\eta,t)$ as the subroutine is the same as in Theorem \ref{th:Complexity}, subject to the adjustment of constant factors. 

%%%%%Away-Step FW%%%%%%%%%%%%%%%%
\subsection{Away-Step Variant}
In this section we consider a particular case of the problem \eqref{eq:Opt} by assuming that the objective function is linear, i.e. $g(x) = \inner{c,x}$ and the set $\setX$ is a polytope in the Euclidean space $\setE=\Rn$. By compactness, the Krein-Milman theorem tells us that $\setX$ is the convex hull of finitely many vertices (extreme points) $\scrU:= \{u_{1},\ldots,u_{q}\}$. This is a relevant scenario of \ac{CndG} methods which received a lot of attention in the literature \cite{Jag13,Cla10}. For instance, the $\ell_{1}$-ball is the convex hull of the signed unit vectors $\scrU=\{\pm e_{i}\vert i\in\{1\ldots,n\}\}.$

Let $\Delta(\scrU)$ denote the set of possible weight vectors $\mu:= (\mu_{u}:u\in\scrU)$ with $\mu_{u}\geq 0$ for all $u\in\scrU$ and $\sum_{u\in\scrU}\mu_{u}=1,\mu_{u}\geq 0$. A measure $\mu^{x}\in\Delta(\scrU)$ is a \emph{vertex representation} of $x$ if $x=\sum_{u\in\scrU}\mu^{x}_{u}u$. Given $\mu\in\Delta(\scrU)$, we define $\supp(\mu):=\{u\in\scrU\vert \mu_{u}>0\}$ and the set of active vertices $\scrU(x):= \{u\in\scrU\vert u\in\supp(\mu^{x})\}$ of point $x\in\scrX$ under the \emph{vertex representation} $\mu^{x}\in\Delta(\scrU)$. We use $I(x):= \{i\in\{1,\ldots,m\}\vert \BB_{i}x=b_{i}\}$ to denote the set of binding constraints at $x$. For a given set $V\subset\scrU$, we let $I(V)=\bigcap_{u\in V}I(u)$.
Given vertex representation, we introduce an additional assumption on the availability of a \emph{vertex linear oracle} \cite{BecSht17}. 
%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{ass:VLO}
The linear minimization procedure in \eqref{eq:LMO}, \eqref{eq:s} returns a vertex solution, i.e. $s_t(x)\in\scrU$ for all $x\in\setX$.
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
Similar to other away-step variants of the CndG method, our algorithm needs also a vertex which is as much aligned as possible with the same direction of the gradient vector at the current position $x$. Such a target vertex is defined as 
\begin{equation}\label{eq:away}
u_t(x)\in\argmax_{u\in\scrU(x)}\left\{t^{-1}F'(x)[u]+\inner{c,u}\right\}.
\end{equation}
At each iteration of the algorithm applied to solve the problem \eqref{eq:potential}, we assume that the iterate $x^{k}$ is represented as a convex combination of active vertices $x^{k}=\sum_{u\in\scrU}\mu^{k}_{u}u$, where $\mu^{k}\in \Delta(\scrU)$. In this case, the sets $U^{k}= \scrU(x^{k})$ and the carrying measure $\mu^{k}=\mu^{x^{k}}$ provide a compact representation of $x^{k}$. The $\ASCG$ scheme updates the representation $(U^{k},\mu^{k})$ via the \emph{vertex representation updating} (VRU) scheme, as defined in \cite{BecSht17}. A single iteration of $\ASCG$ can perform two different updating steps:
\begin{enumerate}
\item \emph{Forward Step}: This update is constructed in the same way as in $\CG$. 
\item \emph{Away Step}: This is a correction step in which the weight of a single vertex is reduced, or even nullified. Specifically, the away step regime builds on the following ideas: Let $x\in\setX$ be the current position of the algorithm with vertex representation $x=\sum_{u\in\scrU}\mu^{x}_{u}u$. Pick $u_t(x)$ as in \eqref{eq:away}. Define the \emph{away direction} 
\begin{equation}\label{eq:vAS}
v_{\AS}(x):= x-u_t(x),
\end{equation}
 and apply the step size $\alpha>0$ to produce the new point 
\begin{align*}
x^{+}_{\alpha}&=x+\alpha v_{\AS}(x)
&=(x-\mu_{u(x)}u(x))(1+\mu^{x}_{u(x)})+(\mu_{u(x)}-t(1-\mu^{x}_{u(x)}))u(x)\\
=\sum_{u\in\scrU(x)\setminus\{u_t(x)\}}(1+\alpha)\mu^{x}_{u}u+\left(\mu^{x}_{u_t(x)}(1+\alpha)-\alpha\right)u_t(x).
\end{align*}
Choosing $\alpha\equiv \bar{\alpha}(x):=\frac{\mu^{x}_{u_t(x)}}{1-\mu^{x}_{u_t(x)}}$ eliminates the vertex $u=u_t(x)$ from the support of the current point $x$ and leaves us with the new position
$x^{+}=x^{+}_{\bar{\alpha}(x)}=\sum_{u\in\scrU(x)\setminus\{u_t(x)\}}\frac{\mu^{x}_{u_t(x)}}{1-\mu^{x}_{u_t(x)}}u$. This vertex removal is called a \emph{drop step.}
\end{enumerate}
To construct a feasible method, we need to impose bounds on the step-size. To that end, define 
\begin{equation}\label{eq:bart}
\bar{\alpha}(x):= \left\{\begin{array}{cc} 
1 & \text{if a Forward Step is performed},\\
\frac{\mu_{u_t(x)}}{1-\mu_{u_t(x)}} & \text{if an Away Step is performed,}
\end{array}\right.
\end{equation}
where $\{\mu_{u}\}_{u\in\scrU}\in\Delta(\scrU)$ is a given vertex representation of the current point $x$, and $u_t(x)$ is the target state identified under the away-step regime \eqref{eq:away}.
%%%%%%%%%%%
%%%%%%ASFWGSC%%%%%%
%=== Away Step FW algorithm==========
%\begin{wrapfigure}{r}{0.56\textwidth}
%\vspace{-0.8cm}
%\begin{minipage}{0.55\textwidth}
\begin{algorithm}[t]
	\caption{$\ASCG(x^{0},\eps,t)$}
	\label{alg:ASCG}
	\begin{algorithmic}
		\State {\bfseries Input: } $(x^{0},t)\in\setC\times(0,\infty)$ initial state such that $\mu^{0}_{u}=0$ for all $u\in\scrU\setminus \{x^{0}\}$ and $U^{0}=\{x^{0}\}$; $\eps>0$ accuracy level.
		\For{$k=0,1,\ldots$}
		\If{$\gap_{t}(x^{k})>\eps$}
			\State Set $s^k=s_t(x^{k}),u^k=u_t(x^{k})$ (see \eqref{eq:s} and \eqref{eq:away})\;
			\State Set $v_{\AS}(x^k)=x^k-u^k$, and $v_{\FW}(x^k)=s^k-x^k$\;
			\If{$t^{-1}F'(x^k)[s^{k}-x^{k}]+\inner{c,s^{k}-x^{k}}\leq t^{-1}F'(x^k)[x^{k}-u^{k}]+\inner{c,x^{k}-u^{k}}$}
				\State Set $v^k=v_{\FW}(x^k)$
			\Else
			\State Set $v^k=v_{\AS}(x^k)$
		\EndIf
		\State Set $\ce_{k}=\norm{v^{k}}_{x^{k}}, \bar{\alpha}_{k}\equiv \bar{\alpha}(x^{k})$ defined in \eqref{eq:bart}\;
		\State Find $\alpha_k=\argmin_{\alpha\in[0,\bar{\alpha}_{k}]}\left\{ \alpha (t^{-1}F'(x^k)[v^{k}]+\inner{c,v^{k}})+ t^{-1}\omega_{\ast}(\alpha\ce_{k})\right\}$\;
		\State Update $x^{k+1}=x^k+\alpha_{k}v^k$
		\If{ $v^k=v_{\FW}(x^k)$}
			\State Update $U^{k+1}=U^{k}\cup\{s^k\}$
		\Else
			\If {$v^k=v_{\AS}(x^{k})$ and $\alpha_{k}=\bar{\alpha}_{k}$}
				\State Update $U^{k+1}=U^{k}\setminus\{u^k\}$ and $\mu^{k+1}$ via the VRU of \cite{BecSht17}.
			\Else 
				\State Update $U^{k+1}=U^k$
			\EndIf
		\EndIf
		\Else
			\State Return $x^{k}$.
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}
%\end{minipage}
%\vspace{-0.2cm}
%\end{wrapfigure}
%============================
%%%%%%%%%%%%%%%%
For the complexity analysis of $\ASCG$, we introduce some convenient notation. Define the vector field $v_t:\setX\to\setE$ by
\begin{equation}\label{eq:thatsv}
v_t(x):= \left\{\begin{array}{cc} 
s_t(x)-x& \text{ if a Forward Step is performed,}\\ %v_{\FW}(x)
x-u_t(x) & \text{if an Away Step is performed.} %v_{\AS}(x)
\end{array}\right.
\end{equation}
We further redefine $\ce_{t}(x):=\norm{v_t(x)}_{x}$, and the modified gap function is 
\begin{align*}
G_t(x)&:=t^{-1}F'(x)[-v_{t}(x)]+\inner{c,-v_{t}(x)}\\
&=\max\left\{t^{-1}F'(x)[x-s_{t}(x)]+\inner{c,x-s_{t}(x)},t^{-1}F'(x)[u_{t}(x)-x]+\inner{c,u_{t}(x)-x}\right\}.
\end{align*}
One observes that $G_t(x)\geq\gap_{t}(x)\geq 0$ for all $x\in\dom F\cap\setX$. 

The construction of our step size policy is based on an optimization argument, similar to the one used in the construction of the $\CG$ algorithm. On a high level, the main difference is that the standard gap $\gap_{t}(x)$ is substituted with the modified gap $G_t(x)$.
Recall that if $\alpha\in(0,\min\{1,1/\ce_{t}(x)\})$, we get from eq. \eqref{eq:descent}
$$
F(x+\alpha v_t(x))\leq F(x)+\alpha F'(x)[v_t(x)]+\omega_{\ast}(\alpha\ce_{t}(x)).
$$
Together with the linearity of $g=\inner{c,x}$, this implies 
\begin{equation}
V_{t}(x+\alpha v_t(x))\leq V_{t}(x)-\alpha G_t(x)+t^{-1}\omega_{\ast}(\alpha\ce_{t}(x)).
\label{eq:V_t_progress_AS}
\end{equation}
The stepsize $\alpha_k$ in $\ASCG$ is obtained by the minimization of the r.h.s. of the above inequality in $\alpha$ on the interval $[0,\bar{\alpha}_{k}]$, where $\bar{\alpha}_{k} = \bar{\alpha}(x^{k})$ is defined in \eqref{eq:bart}. Thus, we observe that $\alpha_k = \min\{\bar{\alpha}(x^{k}),\alpha_{t}(x^{k})\}$, where the function $\alpha_{t}(x)$ is defined as (cf. \eqref{eq:alpha})
\begin{equation}\label{eq:alpha_AS}
\alpha_{t}(x):=\min\left\{1,\frac{tG_{t}(x)}{\ce_{t}(x)(\ce_{t}(x)+tG_{t}(x))}\right\}.
\end{equation}
Revisiting the proof of Proposition \ref{prop:Delta} with the change $\gap_t(x^{k}) \to G_t(x^{k})$, we see that in the regime $\alpha_k = \alpha_{t}(x^{k})$, we guarantee that $V_{t}(x^{k+1}_{t}) \leq V_{t}(x^{k}_{t})$. 
In the opposite case, when $\alpha_k = \bar{\alpha}(x^{k})$ there are, in turn, two options: a) Forward Step is applied; and b) Away Step is applied. In the case a), we have $\bar{\alpha}(x^{k})=1$ and, thus, $\alpha_k = \min\{\bar{\alpha}(x^{k}),\alpha_{t}(x^{k})\} = \min\{1,\alpha_{t}(x^{k})\}\stackrel{\eqref{eq:alpha_AS}}{=}\alpha_{t}(x^{k})$, and we again see that $V_{t}(x^{k+1}_{t}) \leq V_{t}(x^{k}_{t})$. In the case b), we also have  $V_{t}(x^{k+1}_{t}) \leq V_{t}(x^{k}_{t})$ since the r.h.s. of \eqref{eq:V_t_progress_AS} is a non-positive decreasing function of $\alpha$ for $\alpha \in [0,\alpha_{t}(x)]$ and in the case b) $\bar{\alpha}(x^{k}) \leq \alpha_{t}(x^{k})$. Thus, we observe that $\ASCG$ generates a non-increasing sequence of values $\{V_{t}(x^{k}_{t})\}_{k\geq 0}$, from which we conclude that the whole sequence $\{x^{k}_{t}\}_{k\geq 0}$ belongs to the level set $\scrS(t,x^{0}_{t})=\{ x \in \dom F \cap \setX \vert V_{t}(x)\leq V_{t}(x^{0}_{t})\}$. By \cite[Lemma 3]{DvuShtSta22}, we obtain that $\scrS(t,x_t^0)$ is compact and the quantity $\tau_t = \min_{x \in \scrS(t,x^{0}_{t})} t^{-1}\nabla^2 F(x)$ is well defined and positive. Thus, since $g(x)$ is linear, by the optimality condition for the function $V_t(x)$, we have 
\begin{equation}
\label{eq:strong_convexity}
V_t(x) - V_t(z^*(t)) \geq \frac{\tau_t}{2}\norm{x-z^*(t)}_2^2, \quad x \in \scrS(t,x^{0}_{t}).
\end{equation}  
%
To formulate the main theoretical result for the $\ASCG$, we need a technical angle condition. Since $\setX$ is a polytope, it admits the explicit representation $\setX = \{x\in\Rn\vert {\mathbf B} x\leq b\}$, where ${\mathbf B}\in\R^{m\times n}$ and $b\in\R^{m}$. We use $I(x):= \{i\in\{1,\ldots,m\}\vert {\mathbf B}_{i}x=b_{i}\}$ to denote the set of binding constraints at $x$. For a given set $V\subset\scrU$, we let $I(V)=\bigcap_{u\in V}I(u)$.
\begin{lemma}[Corollary 3.1, \cite{BecSht17}]
\label{lem:Error}
For any $x\in\setX\setminus\setX^{\ast}$ with support $\scrU(x)$, we have 
\begin{equation}
\max_{u\in\scrU(x),w\in\scrU}\inner{t^{-1}F'(x)+c,u-w}\geq\frac{\Omega_{\setX}}{\abs{\scrU(x)}}\max_{x^{\ast}\in\setX^{\ast}}\frac{\inner{t^{-1}F'(x)+c,x-x^{\ast}}}{\norm{x-x^{\ast}}},
\end{equation}
where 
\begin{align*}
&\zeta:= \min_{u\in\scrU,i\in\{1,\ldots,m\}:b_{i}>({\mathbf B} u)_{i}}(b_{i}-{\mathbf B}_{i}u),\;\varphi:=\max_{i\in\{1,\ldots,m\}\setminus I(x)}\norm{{\mathbf B}_{i}},\text{ and }\Omega_{\setX}:= \frac{\zeta}{\varphi}.
\end{align*}
\end{lemma}
%
Given the above preliminaries, we are now in a position to formulate the main complexity result for the Algorithm \ref{alg:ASCG} that constructs a sequence $\{x^{k}_{t}\}_{k\in\N}$. Note that in the simplified setting of this section $\Omega_{g}:=\max_{x,y\in\setX}\abs{\inner{c,x-y}} \leq \norm{c} {\rm diam} (\setX)$.
%
\begin{proposition}\label{prop:Delta_AS}
Algorithm $\ASCG(x^{0}_{t},\eta,t)$ requires at most 
\begin{equation}
\label{eq:ASCG_delta_compl}
\widehat{N}(x^{0}_{t},\eta,t):=\lceil 5.3(\nu+t\Delta_{t}(x^{0}_{t})+t\Omega_{g})\log(10.6t\Delta_{t}(x^{0}_{t}))\rceil+\lceil\frac{2}{\theta } \log \frac{\Delta_{t}(x^{0}_{t})}{\eta} \rceil
\end{equation}
iterations, in order to reach a point satisfying $\Delta_{t}(x^{k}_{t})\leq \eta$. Here $ \theta := \min\left\{\frac{1}{2}, \frac{\Omega}{4\diam(\setX)}, \frac{\Omega^{2}\tau_{t}}{96}\frac{t}{(\nu+t\Omega_{g})^{2}}\right\}$ and $\Omega = \frac{\Omega_{\setX}}{|\scrU|}$. Moreover, it holds that $\widehat{N}(x^{0}_{t},\eta,t) \leq 2 N(x^{0}_{t},\eta,t)$, where $N(x^{0}_{t},\eta,t)$ is defined in Proposition \ref{prop:Delta}.
\end{proposition}
%
\begin{proposition}\label{prop:gap_AS}
Given $\eta,t>0$, let $\widehat{R}(x^{0}_t,\eta,t)$ be the first iterate $k$ of Algorithm $\ASCG(x^{0}_t,\eta,t)$ satisfying $\gap_{t}(x^{k}_t)\leq\eta$. Then 
\begin{equation}
\label{eq:ASCG_gap_compl}
\widehat{R}(x^{0}_t,\eta,t)\leq \lceil 5.3(\nu+t\Delta_{t}(x^{0}_t)+t\Omega_{g})\log(10.6t\Delta_{t}(x^{0}_t))\rceil+\lceil \frac{192(\nu+t\Omega_{g})^{2}}{t\tau_t \Omega} \log \frac{12 Delta_{t}(x^{0}_{t}) \cdot (\nu+t\Omega_{g})^{2}}{t \eta^2}\rceil,
\end{equation}
where $\Omega$ is defined in Proposition \ref{prop:Delta_AS}.
Moreover, it holds that $\widehat{R}(x^{0}_{t},\eta,t) \leq 2 R(x^{0}_{t},\eta,t)$, where $R(x^{0}_{t},\eta,t)$ is defined in Proposition \ref{prop:gap}.
\end{proposition}


==> inexactLMO.tex <==
%%----------------------------------------------------------------------
%%% Analysis - Inexact - now also with multiplicative error
%----------------------------------------------------------------------
% !TEX root = ./SDP_main.tex
%
In this appendix we give the missing proofs of the theoretical statements in Sections \ref{sec:extensions} and \ref{sec:inexact-path-following}.  
Consider the function $\tilde{\ce}_{t}(x):=\norm{\tilde{s}_{t}(x)-x}_{x}$, where $\tilde{s}_{t}(x)$ is any member of the set $\scrL^{(\delta,\theta)}_{g}(\frac{1}{t}\nabla F(x))$ (cf. Definition \ref{def:ILMO}). It is easy to see that \ref{lem:e-bound} translates to the case with inexact oracle feedback as
\begin{equation}\label{eq:tildee-bound}
t^{-1}\tilde{\ce}_{t}(x)\leq \nu/t+\widetilde{\gap}_{t}(x)+\Omega_{g}.
\end{equation}
Moreover, one can show that 
\begin{equation}\label{eq:e-LB}
\tilde{\ce}_{t}(x)\geq \frac{t}{\sqrt{\nu}}\abs{\widetilde{\gap}_{t}(x)-\Omega_{g}}.
\end{equation}
\SH{why is the last equality true with absolute value, should it not be $|\widetilde{\gap}_{t}(x)|-\Omega_{g}$?}

\subsection{Proof of Proposition \ref{prop:DeltaInexact}}
The proof of this proposition mimics the proof of the exact regime (cf. Proposition \ref{prop:Delta}), with some important twists. We split the analysis into two phases, bound the maximum number of iterations the algorithms can spend on these phases, and add these numbers up to obtain the worst-case upper bound.% reported in \ref{prop:DeltaInexact}.

First, for a round $k$ of $\texttt{ICG}(x,t,\eta,\delta,\theta)$, we use the abbreviations  
$$
\tilde{s}_{t}^{k}=\tilde{s}_{t}(x^{k}_{t}),\; \tilde{\ce}_{t}^{k}\equiv\norm{\tilde{s}_{t}^{k}-x^{k}_{t}}_{x^{k}_{t}},\; \tilde{G}^{k}_{t}\equiv \widetilde{\gap}_{t}(x^{k}_{t}),\;\tilde{\alpha}_{t}^{k}\equiv \tilde{\alpha}_{t}(x^{k}_{t}).
$$
We further redefine the phases as $\K_{I}(t):=\{k\in\N\vert \widetilde{\gap}_{t}(x^{k}_{t})>\ca_{t}\}$ (phase I) and $\K_{II}(t):=\{k\in\N\vert\widetilde{\gap}_{t}(x^{k}_{t})\leq \ca_{t}\}$ (phase II), where $\ca_{t}:=\frac{\nu}{t}+\Omega_{g}$.



Note that in the analysis we use the inequality $\Delta_{t}(x^{k}_{t}) >\eta + \theta$ since our goal is to estimate the number of iterations to achieve $\Delta_{t}(x^{k}_{t}) \leq \eta + \theta$. Moreover, if the stopping condition $\widetilde{\gap}_{t}(x^{k}_{t}) \equiv \tilde{G}^{k}_{t} \leq \eta \delta $ holds, we obtain by the definition of the \ac{ILMO} and inequality \eqref{eq:relationGap} that 
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_0}
\eta \delta \geq \widetilde{\gap}_{t}(x^{k}_{t})\geq\delta(\gap_{t}(x^{k}_{t})-\theta)\geq \delta(\Delta_{t}(x^{k}_{t})-\theta),
\end{equation}
which implies that $\Delta_{t}(x^{k}_{t}) \leq \eta + \theta$. Thus, in the analysis we also use the inequality $\tilde{G}^{k}_{t} > \eta \delta >0$.
%\widetilde{\gap}_{t}(x^{k}_{t})\equiv\tilde{G}^{k}_{t}\geq\delta(\gap_{t}(x^{k}_{t})-\theta)\equiv\delta(G^{k}_{t}-\theta) \geq \delta(\Delta_{t}(x^{k}_{t})-\theta)
%the inequality $\tilde{G}^{k}_{t} > \eta \delta >0$ which holds since the stopping condition is not yet achieved, and . 

\paragraph{Analysis for Phase I} 
Consider $k\in\K_{I}(t)$. 
%To reduce notational clutter even further, we also set $\delta_{t}\equiv \delta$ and $\theta_{t}\equiv\theta$ for the remainder of the analysis. 
%For such iterations, we have $\tilde{G}^{k}_{t} > \frac{\nu}{t}+\Omega_{g}$. %$\frac{t\tilde{G}^{k}_{t}}{\nu+t\tilde{G}^{k}_{t}+t\Omega_{g}}>\frac{1}{2}$. 
Combining the condition $\tilde{G}^{k}_{t} > \frac{\nu}{t}+\Omega_{g}$ of this phase with \eqref{eq:e-LB}, we deduce \sh{from \eqref{eq:e-LB}} that $\tilde{\ce}^{k}_{t}\geq \sqrt{\nu}\geq 1$. This in turn implies $\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}_{t}(\tilde{\ce}^{k}_{t}+t\tilde{G}^{k}_{t})}<\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}+t \tilde{G}^{k}_{t}}<1$. Hence, at this iteration algorithm $\texttt{ICG}(x,t,\eta,\delta,\theta)$ chooses the step size $\tilde{\alpha}_{t}^{k}=\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}_{t}(\tilde{\tilde{\ce}}^{k}_{t}+t\tilde{G}^{k}_{t})}$. The per-iteration reduction of the potential function can then be estimated just as in the derivation of \eqref{eq:V_t_progress_1}:
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_1}
V_{t}(x^{k+1}_{t})\leq V_{t}(x^{k}_{t})-\frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}_{t}^{k}}\right).
\end{equation}
Note that the r.h.s. is well-defined since $\tilde{G}^{k}_{t} > \eta \delta >0$ as the stopping condition is not yet achieved. The above inequality, using the definition of the potential function gap as $\Delta_{t}(x^{k}_{t})=V_{t}(x^{k}_{t})-V_{t}(z^{\ast}(t))$, readily yields $\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}_{t}}\right)$ and, in turn, that $\{\Delta_{t}(x^{k}_{t})\}_{k\in\K_{I}(t)}$ is monotonically decreasing.

Since $k\in\K_{I}(t)$, we have that $\frac{t\tilde{G}^{k}_{t}}{\nu+t\tilde{G}^{k}_{t}+t\Omega_{g}}>\frac{1}{2}$. Together with \eqref{eq:tildee-bound}, this implies 
\[
\frac{t\tilde{G}_{t}^{k}}{\tilde{\ce}^{k}_{t}}\geq\frac{\tilde{G}^{k}_{t}}{\nu/t+\tilde{G}_{t}^{k}+\Omega_{g}}=\frac{t\tilde{G}^{k}_{t}}{\nu+t\tilde{G}_{t}^{k}+t\Omega_{g}}>\frac{1}{2}.
\]
Using the monotonicity of $\omega(\cdot)$ and that $\omega(\tau) \geq \frac{\tau}{5.3}$ for $\tau\geq 1/2$ \cite[Prop. 1]{ZhaFre20}, we further obtain
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_2}
\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}_{t}}\right) \geq \frac{\tilde{G}^{k}_{t}}{5.3(\nu+t\Omega_{g}+t\tilde{G}_{t}^{k})}.
\end{equation}
By our definition of the inexact oracle, inequalities \eqref{eq:relationGap} and $\Delta_{t}(x^{k}_{t}) > \eta + \theta$, we see that
\[
\tilde{G}^{k}_{t} \equiv\widetilde{\gap}_{t}(x^{k}_{t})\geq\delta(\gap_{t}(x^{k}_{t})-\theta) \geq \delta(\Delta_{t}(x^{k}_{t})-\theta) > \eta >0. %\equiv\delta(G^{k}_{t}-\theta)
\]
%By our definition of the inexact oracle, inequalities \eqref{eq:relationGap} and $\Delta_{t}(x^{k}_{t}) \geq 0$, and our assumption that $\theta < \frac{1}{\delta}\left(\frac{\nu}{t}+\Omega_g \right)$, we see that
%\[
%\widetilde{\gap}_{t}(x^{k}_{t})\equiv\tilde{G}^{k}_{t}\geq\delta(\gap_{t}(x^{k}_{t})-\theta)\equiv\delta(G^{k}_{t}-\theta) \geq \delta(\Delta_{t}(x^{k}_{t})-\theta) > - \frac{\nu}{t}-\Omega_g \equiv -\ca_{t}.
%\]
Combining this, \eqref{eq:ILMO_prop_Delta_proof_2}, and the fact that the function $x\mapsto \frac{x}{a+tx}$ is strictly increasing for $a,t >0$ and $x>0$, we obtain
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_3}
\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{\delta(\Delta_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\Delta_{t}(x^{k}_{t})-\theta)+\nu+t\Omega_{g}]}  \geq \frac{\delta(\Delta_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g}]},
\end{equation}
where in the last inequality we used that $\Delta_{t}(x^{k}_{t})> \eta + \theta \geq \theta$ and the monotonicity of $\{\Delta_{t}(x^{k}_{t})\}_{k\in\K_{I}(t)}$.

Rearranging the terms and defining $q:=\frac{\delta}{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}$, which we know to be in $(0,1)$ since $\nu\geq 1$ and $\Delta_{t}(x^{0}_{t}) > \eta + \theta$, it follows from the previous display that \SH{the numbering here is wrong, it should be the numbering within phase I and not of the iterate, also why is it true for $x_t^0$?}
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_4}
\Delta_{t}(x^{k+1}_{t})\leq  \Delta_{t}(x^{k}_{t}) (1-q) + q \theta \leq  \Delta_{t}(x^{0}_{t})(1-q)^{k}+\theta \leq \exp(-kq)\Delta_{t}(x^{0}_{t})+\theta.
\end{equation}

On the other hand, we have
$$
\Delta_{t}(x^{k}_{t}) \geq \Delta_{t}(x^{k}_{t}) - \Delta_{t}(x^{k+1}_{t}) \geq \frac{\tilde{G}^{k}_{t}}{5.3(\nu+t\Omega_{g}+t\tilde{G}_{t}^{k})}>\frac{1}{10.6 t }
$$
since $\frac{t\tilde{G}^{k}_{t}}{\nu+t\tilde{G}^{k}_{t}+t\Omega_{g}}>\frac{1}{2}$ for $k\in\K_{I}(t)$.
Moreover, we know that $\Delta_{t}(x^{k}_{t}) > \eta + \theta$, which gives us in combination with \eqref{eq:ILMO_prop_Delta_proof_4} 
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_5}
\max\left\{\frac{1}{10.6 t }, \eta + \theta \right\} \leq \Delta_{t}(x^{k}_{t}) \leq \exp(-kq)\Delta_{t}(x^{0}_{t})+\theta.
\end{equation}
Solving w.r.t. $k$, we see that the number of iterations $k\in\K_{I}(t)$ is bounded as 
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_6}
K_{t}(x_{t}^{0}): = \left\lceil \frac{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}{\delta}\log\left( \min\left\{\frac{10.6 t \Delta_{t}(x^{0}_{t})}{(1-10.6 t \theta)_+}, \frac{\Delta_{t}(x^{0}_{t})}{\eta} \right\}\right)  \right\rceil.
\end{equation}






%%%%%%%%%%%%%%%%%%%%%%%%% analysis before 01/09/23
%Using this in the upper bound \ref{eq:upperV}, we see that 
%\begin{align*}
%V_{t}(x^{k+1}_{t})&\leq V_{t}(x^{k}_{t})-\frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}_{t}^{k}}\right)\\
%&\leq V_{t}(x^{k}_{t})-\frac{\tilde{G}^{k}_{t}}{5.3(\nu+t\Omega_{g}+t\tilde{G}_{t}^{k})}.
%\end{align*}
%Using the definition of the potential function gap as $\Delta_{t}(x^{k}_{t})=V_{t}(x^{k}_{t})-V_{t}(z^{\ast}(t))$, we have 
%$$
%-\Delta_{t}(x^{k}_{t})\leq \Delta_{t}(x^{k+1}_{t})-\Delta_{t}(x^{k}_{t})\leq -\frac{\tilde{G}^{k}_{t}}{5.3(\nu+t\Omega_{g}+t\tilde{G}_{t}^{k})}<-\frac{1}{10.6 t }
%$$
%since $\frac{t\tilde{G}^{k}_{t}}{\nu+t\tilde{G}^{k}_{t}+t\Omega_{g}}>\frac{1}{2}$. This proves that $\Delta_{t}(x^{k}_{t})$ is a decreasing sequence on $\K_{I}(t)$. Furthermore, we can ensure that $\Delta_{t}(x^{k}_{t})\geq\theta$, by setting $\theta<\frac{1}{10.6t}$. Since $\gap_{t}(x)\geq\Delta_{t}(x)$, this implies additionally that $\gap_{t}(x^{k}_{t})\geq\theta$. 
%
%Recall the definition of the inexact oracle with multiplicative errors states that 
%$$
%\widetilde{\gap}_{t}(x^{k}_{t})\equiv\tilde{G}^{k}_{t}\geq\delta(\gap_{t}(x^{k}_{t})-\theta)\equiv\delta(G^{k}_{t}-\theta).
%$$
%Just as in the exact oracle regime, we obtain from this bound the monotone decrease of the potential function gap as 
%$$
%\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{\delta(\gap_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\gap_{t}(x^{k}_{t})-\theta)+\nu+t\Omega_{g}]}.
%$$
%Continuing from this line, we thus obtain the successive lower bounds
%\begin{align*}
%\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})&\geq  \frac{\delta(\gap_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\gap_{t}(x^{k}_{t})-\theta)+\nu+t\Omega_{g}]}\\
 %& \geq \frac{\delta(\Delta_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\Delta_{t}(x^{k}_{t})-\theta)+\nu+t\Omega_{g}]} \\
%&\geq \frac{\delta(\Delta_{t}(x^{k}_{t})-\theta)}{5.3[t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g}]}
%\end{align*}
%where in the last inequality we have used the monotone decrease of the sequence $\{\Delta_{t}(x^{k}_{t})\}_{k\in\K_{I}(t)}$. Rearranging expressions, we thus obtain 
%$$
%\frac{\delta\theta}{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}+\Delta_{t}(x^{k}_{t})\left[1-\frac{\delta}{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}\right]\geq \Delta_{t}(x^{k+1}_{t}).
%$$
%Setting $q:=\frac{\delta}{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}$, which we know to be in $(0,1)$ since $\nu\geq 1$, it follows from the penultimate display 
%$$
%\Delta_{t}(x^{k}_{t})\leq\Delta_{t}(x^{0}_{t})(1-q)^{k}+\theta\leq \exp(-kq)\Delta_{t}(x^{0}_{t})+\theta.
%$$
%At the same time, for $k\in\K_{I}(t)$, we know that
%$$
%\Delta_{t}(x^{k}_{t})\geq\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{1}{10.6t}.
%$$
%Combining this lower bound with the established upper bound, we can estimate the number of iterations we spend in phase I to be at most
%$$
%\left\lceil \frac{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}{\delta}\log\left(\frac{10.6t\Delta_{t}(x^{0}_{t})}{1-10.6t\theta}\right)\right\rceil.
%$$









\paragraph{Analysis for Phase II}
Consider $k\in\K_{II}(t)$, which means that $\tilde{G}_{t}^{k}\leq \frac{\nu}{t}+\Omega_{g}$. There are two cases we need to consider, depending on the step size $\tilde{\alpha}_{t}^{k}$. 

First, assume that $\tilde{\alpha}_{t}^{k}=1$. Then $t\tilde{G}_{t}^{k}\geq\tilde{\ce}^{k}_{t}(\tilde{\ce}_{t}^{k}+t\tilde{G}_{t}^{k})$, which implies $\tilde{\ce}_{t}^{k}\in(0,1)$. From there we conclude that $\tilde{G}_{t}^{k}\geq \frac{(\tilde{\ce}_{t}^{k})^{2}}{t(1-\tilde{\ce}_{t}^{k})}$, and, by \eqref{eq:upperV} and \eqref{eq:boundomega}, that
\begin{align*}
V_{t}(x^{k+1}_{t})&\leq V_{t}(x^{k}_{t})-\tilde{G}_{t}^{k}+\frac{1}{t}\omega_{\ast}(\tilde{\ce}_{t}^{k})\\
&\leq V_{t}(x^{k}_{t})-\tilde{G}_{t}^{k}+\frac{1}{t}\frac{(\tilde{\ce}^{k}_{t})^{2}}{2(1-\tilde{\ce}_{t}^{k})}\\
&\leq V_{t}(x^{k}_{t})-\frac{\tilde{G}^{k}_{t}}{2}.
\end{align*}
Therefore, using again that $\tilde{G}_{t}^{k}\leq \frac{\nu}{t}+\Omega_{g}$, we have
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_7}
\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{\tilde{G}^{k}_{t}}{2} \geq\frac{(\tilde{G}^{k}_{t})^{2}}{2(\nu/t+\Omega_{g})}\geq \frac{t(\tilde{G}^{k}_{t})^{2}}{12(\nu+t\Omega_{g})^{2}}.
\end{equation}
In particular, we see again that $\Delta_{t}(x^{k}_{t})$ is monotonically decreasing since $\tilde{G}^{k}_{t} > \eta \delta >0$. 

Consider now the case where $\tilde{\alpha}_{t}^{k}<1$, i.e.,  $\tilde{\alpha}_{k}=\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}^{k}_{t}(\tilde{\ce}^{k}_{t}+t\tilde{G}^{k}_{t})}$.
Then, using this stepsize, just as in the derivation of \eqref{eq:V_t_progress_1} and \eqref{eq:ILMO_prop_Delta_proof_1}, we get 
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_8}
V_{t}(x^{k+1}_{t})\leq V_{t}(x^{k}_{t})-\frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}_{t}^{k}}\right).
\end{equation}
Again, since $\tilde{G}_{t}^{k}\leq \frac{\nu}{t}+\Omega_{g}$ for $k\in\K_{II}(t)$, we have $\frac{\tilde{G}^{k}_{t}}{\tilde{G}^{k}_{t}+\nu/t+\Omega_{g}} \leq \frac{1}{2}$. 
Using the monotonicity of $\omega(\tau)$, inequality \eqref{eq:tildee-bound}, and that $\omega(\tau) \geq \frac{\tau^2}{3}$ for $\tau\leq 1/2$ \cite[Prop. 1]{ZhaFre20},  we can develop the bound
%Using monotonicity of the function $t\mapsto \omega(t)$ on its domain, inequalities \eqref{eq:tildee-bound} and \eqref{}, we can develop the bound 
$$
\frac{1}{t}\omega\left(\frac{t\tilde{G}^{k}_{t}}{\tilde{\ce}_{t}^{k}}\right)=\frac{1}{t}\omega\left(\frac{\tilde{G}^{k}_{t}}{\tilde{\ce}_{t}^{k}/t}\right)\geq \frac{1}{t}\omega\left(\frac{\tilde{G}^{k}_{t}}{\tilde{G}^{k}_{t}+\nu/t+\Omega_{g}}\right)\geq\frac{1}{3t}\left(\frac{\tilde{G}^{k}_{t}}{\tilde{G}^{k}_{t}+\nu/t+\Omega_{g}}\right)^{2}.
$$
This and \eqref{eq:ILMO_prop_Delta_proof_8}, again by $\tilde{G}_{t}^{k}\leq \frac{\nu}{t}+\Omega_{g}$, implies that also in this regime we obtain the estimate 
\begin{equation}
\label{eq:ILMO_prop_Delta_proof_9}
\Delta_{t}(x^{k}_{t})-\Delta_{t}(x^{k+1}_{t})\geq \frac{t(\tilde{G}^{k}_{t})^{2}}{12(\nu+t\Omega_{g})^{2}}.
\end{equation}
As we see, the above inequality holds on the whole phase II, both when $\tilde{\alpha}_{t}^{k}<1$ and when $\tilde{\alpha}_{t}^{k}=1$. In particular, since $\tilde{G}^{k}_{t} > \eta \delta >0$, the above inequality implies that the sequence $\{\Delta_{t}(x^{k}_{t})\}_{k\in\K_{II}(t)}$ is monotonically decreasing, which combined with the analysis of phase I means that the whole sequence $\{\Delta_{t}(x^{k}_{t})\}_{k}$ is monotonically decreasing.

\paragraph{Finalising the proof}
Let $K$ denote the number in the r.h.s. of \eqref{eq:prop:DeltaInexact} and let $\texttt{ICG}(x,t,\eta,\delta,\theta)$ be run for $K$ iterations. Let $N_{t}(x_{t}^{0}) := \left \lceil \frac{12(\nu+t\Omega_{g})^{2}}{t\delta^{2}}\left(\frac{1}{\eta}-\frac{1}{\Delta_{t}(x^{0}_{t})-\theta}\right)_{+}\right\rceil$.
Then, from the expression for $K$ and the analysis of phase I, we know that at least $N_{t}(x_{t}^{0})+1$ iterations belong to the phase II. If at some of these iterations, we have $\Delta_{t}(x^{k}_{t})\leq\eta+\theta$, the result of the proposition follows. Thus, we assume that for the whole phase II  $\Delta_{t}(x^{k}_{t})>\eta+\theta>\theta$. 
Let $k_{1}(t)<k_{2}(t)<\ldots<k_{N_{t}(x_{t}^{0})+1}(t) $ be an increasing enumeration of the iterates in $\K_{II}(t)$. Then, using the monotonicity of the entire sequence $\{\Delta_{t}(x^{k}_{t})\}_{k}$, calling $\Delta_{t}^{j}\equiv\Delta(x^{k_{j}(t)}_{t})$, we see from \eqref{eq:ILMO_prop_Delta_proof_9} and \eqref{eq:ILMO_prop_Delta_proof_0} that, for $j=1,\ldots,N_{t}(x_{t}^{0})$,
$$
\Delta^{j}_{t}-\Delta^{j+1}_{t}\geq \Delta^{j}_{t}-\Delta_{t}(x^{k_{j}(t)+1}_{t})\geq \frac{t(\tilde{G}^{\sh{k_{j}(t)}}_{t})^{2}}{12(\nu+t\Omega_{g})^{2}} \geq \frac{t\delta^{2}(\Delta^{j}_{t}-\theta)(\Delta^{j+1}_{t}-\theta)}{12(\nu+t\Omega_{g})^{2}}.
$$
This implies since $\Delta_{t}(x^{k}_{t})>\theta$ for $j=1,\ldots,N_{t}(x_{t}^{0})+1$ that
$$
\frac{1}{\Delta^{j+1}_{t}-\theta}-\frac{1}{\Delta^{j}_{t}-\theta}\geq\frac{t\delta^{2}}{12(\nu+t\Omega_{g})^{2}}, \quad j=1,\ldots,N_{t}(x_{t}^{0}).
$$
Telescoping this expression, we see 
$$
\frac{1}{\Delta^{N_{t}(x_{t}^{0})+1}_{t}-\theta} \geq \frac{N_{t}(x_{t}^{0}) t\delta^{2}}{12(\nu+t\Omega_{g})^{2}} + \frac{1}{\Delta_{t}(x_{t}^{0})-\theta} \geq \frac{1}{\eta},
$$
which finishes the proof.


%%%%%%%%%%%%%%%%%%%%%%%%%% analysis before 01/09/23
%For the rest of the analysis we assume that $\Delta_{t}(x^{k}_{t})>\theta$ for all $k\in\K_{II}(t)$, since, if not true, we should have already stopped. %We will say later why we can make this assumption without loss of generality for the worst-case complexity analysis. Adopting this convention, it follows that $\Delta_{t}(x^{k}_{t})>\theta$ for all iterations $k$ in the inner loop procedure.\footnote{To wit, if $k\in\K_{II}(t)$, then $k+1$ is either in $\K_{I}(t)$ or in $\K_{II}(t)$. If it belongs to $\K_{I}(t)$, we know the statement is true because $\theta<\frac{1}{10.6t}$. Else, $k\in\K_{II}(t)$, and the statement is true by hypothesis.}
%
%Making this assumption, let $k_{1}(t)<k_{2}(t)<\ldots $ be an increasing enumeration of the iterates in $\K_{II}(t)$. Then, using the monotonicity of the entire sequence $\{\Delta_{t}(x^{k}_{t})\}_{k}$, calling $\Delta_{t}^{j}\equiv\Delta(x^{k_{j}(t)}_{t})$, we see 
%$$
%\Delta^{j}_{t}-\Delta^{j+1}_{t}\geq \Delta^{j}_{t}-\Delta_{t}(x^{k_{j}(t)+1}_{t})\geq \frac{t\delta^{2}(\Delta^{j}_{t}-\theta)(\Delta^{j+1}_{t}-\theta)}{12(\nu+t\Omega_{g})^{2}}.
%$$
%This implies 
%$$
%\frac{1}{\Delta^{j+1}_{t}-\theta}-\frac{1}{\Delta^{j}_{t}-\theta}\geq\frac{t\delta^{2}}{12(\nu+t\Omega_{g})^{2}}.
%$$
%Telescoping this expression, we see 
%$$
%\frac{1}{\Delta^{J}_{t}-\theta}-\frac{1}{\Delta^{0}_{t}-\theta}\geq \frac{J t\delta^{2}}{12(\nu+t\Omega_{g})^{2}}.
%$$
%In order to make $\Delta^{J}_{t}\leq\eta+\theta$, we therefore need at most 
%$$
%\left \lceil \frac{12(\nu+t\Omega_{g})^{2}}{t\delta^{2}}\left[\frac{1}{\eta}-\frac{1}{\Delta_{t}(x^{0}_{t})-\theta}\right]_{+}\right\rceil.
%$$
%iterations in Phase II. 

\subsection{Proof of Proposition \ref{prop:GapInexact}}

%\begin{proof}[Proof of \ref{prop:GapInexact}]
Our analysis concentrates on the behaviour of the algorithm in Phase II since the estimate for number of iterations in Phase I still holds. Here we split the iterates of the set $\K_{II}(t)=\{k_{1}(t),\ldots,k_{p}(t)\}\equiv \{k_{1},\ldots,k_{p}\}$ into two regimes so that $\K_{II}(t)=H_{t}\cup L_{t}$ with $L_{t}:=\{k\in\K_{II}(t)\vert \Delta_{t}(x^{k}_{t})<\theta\}$ and $H_{t}:=\{k\in\K_{II}(t)\vert \Delta_{t}(x^{k})\geq \theta\}$. By monotonicity of the potential function gap, we know that the indices of of $H_{t}$ ('high states') precede those of $L_{t}$ ('low states'). We bound the size of each of these subsets in order to make $\widetilde{\gap}_{t}$ smaller than $\eta\delta$. Since the potential function gap is monotonically decreasing, we can organise the iterates on phase II as $H_{t}=\{k_{1},\ldots,k_{q}\}$ and accordingly, $L_{t}=\{k_{q+1},\ldots,k_{p}\}$ for some $q\in\{1,\ldots,p\}$. 

\paragraph{Bound on $H_{t}$:}  
For $k_{j}(t)\in H_{t}$ we know that 
\begin{equation}\label{eq:DeltaBound}
\Delta_{t}(x^{k_{j}(t)}_{t})-\Delta_{t}(x^{k_{j+1}(t)}_{t})\geq \Delta_{t}(x^{k_{j}(t)}_{t})-\Delta_{t}(x^{k_{j}(t)+1}_{t})\geq \frac{t(\tilde{G}^{k_{j}(t)}_{t})^{2}}{12(\nu+t\Omega_{g})^{2}}.
\end{equation}
Define $d_{j}:=\delta(\Delta_{t}(x^{k_{j}(t)}_{t})-\theta)$ for $j=1,\ldots,q$, so that $d_{j}\geq 0$. Then, we obtain the recursion 
$$
d_{j+1}-d_{j}\leq-\frac{\Gamma^{2}_{j}}{M}
$$
for $j\in\{1,\ldots,q-1\}$ and $\Gamma_{j}\equiv\tilde{G}^{k_{j}(t)}_{t}\geq d_{j}$ and $\frac{1}{M}\equiv \frac{t\delta}{12(\nu+t\Omega_{g})^{2}}$. By \cite[Proposition 4]{ZhaFre20}, we can conclude that 
$$
d_{q}<\frac{M}{q-1}\text{ and }\min\{\Gamma_{1},\ldots,\Gamma_{q}\}<\frac{2M}{q-1}.
$$
Since we know that $\min\{\Gamma_{1},\ldots,\Gamma_{q}\}\geq\delta\eta$, we obtain the bound 
\begin{equation}\label{eq:q}
q\leq \frac{2M}{\delta\eta}+1=\frac{24(\nu+t\Omega_{g})^{2}}{t\delta^{2}\eta}+1.
\end{equation}

\paragraph{Bound on $L_{t}$:} 
On this subset we cannot use the same argument as for the iterates in $H_{t}$, since we cannot guarantee that the sequence $d_{j}$ involved in the previous part of the proof is positive. However, we still know that \eqref{eq:DeltaBound} applies for the iterates in $L_{t}$. If we telescope this expression over the indices $q+1,\ldots,p$, and using the fact that $\Delta_{t}(x^{k_{j}}(t))\in[0,\theta]$, we see that 
\begin{align*}
\theta\geq \Delta_{t}(x_{t}^{k_{q+1}(t)})-\Delta_{t}(x_{t}^{k_{p+1}(t)})&\geq \frac{t(p-q)}{12(\nu+t\Omega_{g})^{2}}\min_{q+1\leq j\leq p}\left(\tilde{G}_{t}^{k_{j}(t)}\right)^{2}\\
&\geq  \frac{t(p-q)\eta^{2}\delta^{2}}{12(\nu+t\Omega_{g})^{2}}
\end{align*}
It follows
\begin{equation}\label{eq:pq}
(p-q)\leq \frac{12\theta(\nu+t\Omega_{g})^{2}}{t\eta^{2}\delta^{2}}.
\end{equation}

\paragraph{Combining the bounds:}
Combining the expressions \eqref{eq:q} and \eqref{eq:pq} together with the bound \eqref{eq:ILMO_prop_Delta_proof_6}, we see that 
\begin{align*}
\tilde{R}_{t}(x^{0}_{t},\eta,\delta,\theta)&= \left\lceil \frac{5.3(t\delta(\Delta_{t}(x^{0}_{t})-\theta)+\nu+t\Omega_{g})}{\delta}\log\left( \min\left\{\frac{10.6 t \Delta_{t}(x^{0}_{t})}{(1-10.6 t \theta)_+}, \frac{\Delta_{t}(x^{0}_{t})}{\eta} \right\}  \right)\right\rceil\\
&+ \left\lceil \frac{12(\nu+t\Omega_{g})^{2}}{t\delta^{2}\eta} \left(2+\frac{\theta}{\eta}\right)\right\rceil+1
\end{align*}
%\end{proof}
defines an upper bound for the length of phase I. 

\subsection{Analysis of the outer loop and proof of Theorem \ref{th:Complexity_inexact}}
We set $\hat{x}_{i}\equiv x^{\tilde{R}_{i}}_{t_{i}}$ the last iterate of procedure $\ICG(x^{0}_{t_{i}},t_{i},\eta_{i},\delta,\theta_{i})$, where $\tilde{R}_{i}$ is at most $R_{\tilde{G},t_{i}}(x^{0}_{t_{i}},\eta_{i},\delta,\theta_{i})$ by \ref{prop:GapInexact}. Therefore, we know that $\widetilde{\gap}_{t_{i}}(\hat{x}_{i})\leq\eta_{i}\delta$, and a-fortiori 
$$
\Delta_{t_{i}}(\hat{x}_{i})\leq \gap_{t_{i}}(\hat{x}_{i})\leq \eta_{i}+\theta_{i}.  
$$
By eq. \ref{eq:g2} and the definition of the $(\delta,\theta_{i})$-\ac{ILMO}, we obtain 
\begin{align*}
g(\hat{x}_{i})-g(z^{\ast}(t_{i}))&\leq\gap_{t_{i}}(\hat{x}_{i})+\frac{1}{t}F'(\hat{x}_{i})[z^{\ast}(t_{i})-\hat{x}_{i}]\\
&\leq \frac{\widetilde{\gap}_{t_{i}}(\hat{x}_{i})}{\delta}+\theta_{i}+\frac{\nu}{t_{i}}\\
&\leq \eta_{i}+\theta_{i}+\frac{\nu}{t_{i}}.
\end{align*}
Hence, using \ref{lem:pathfollowing}, we observe
$$
g(\hat{x}_{i})-\Opt=g(\hat{x}_{i})-g(z^{\ast}(t_{i}))+g(z^{\ast}(t_{i}))-\Opt\leq \eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}.
$$
Since $t_{i}=\frac{2\nu}{\eta_{i}}$ and $\theta_i=\eta_i$, we obtain $g(\hat{x}_{i})-\Opt\leq  3\eta_{i}$. The latter, by the choice of the number of restarts $I$ implies that 
$$
g(\hat{z})-\Opt = g(\hat{x}_{I})-\Opt \leq \eps.
$$

Our next goal is to estimate the total number of inner iterations based on the estimation for the first epoch $i=0$ and summation over epochs $i=1,...,I$. For each epoch we use the estimate from \ref{prop:GapInexact}, which we repeat here for convenience
\begin{align}
\label{eq:IO_outer_proof_2}
\tilde{R}_{t_i}(x^{0}_{t_{i}},\eta_{i},\delta,\theta_{i})&= \left\lceil \frac{5.3(t_{i}\delta(\Delta_{t_{i}}(x^{0}_{i})-\theta_{i})+\nu+t_{i}\Omega_{g})}{\delta}\log\left( \min\left\{\frac{10.6 t_{i} \Delta_{t_{i}}(x^{0}_{t_{i}} )}{(1-10.6 t_{i} \theta_{i})_+}, \frac{\Delta_{t_{i}}(x^{0}_{t_{i}})}{\eta_{i}} \right\} \right) \right\rceil \notag \\
& \hspace{2em} + \left\lceil \frac{12(\nu+t_{i}\Omega_{g})^{2}}{t_{i}\delta^{2}\eta_{i}} \left(2+\frac{\theta_{i}}{\eta_{i}}\right)\right\rceil+1.
\end{align}
We see that we need to estimate the quantities $t_{i}(\Delta_{t_{i}}(x^{0}_{i})-\theta_{i})$ and $\frac{\Delta_{t_{i}}(x^{0}_{t_{i}})}{\eta_{i}}$, which is our next step.
Consider $i\geq 1$ and observe that
\begin{align*}
	V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))&=V_{t_{i}}(x^{0}_{t_{i+1}})-V_{t_{i}}(z^{\ast}(t_{i+1}))\\
	&+\left(\frac{1}{t_{i+1}}-\frac{1}{t_{i}}\right)(F(x^{0}_{t_{i+1}})-F(z^{\ast}(t_{i+1})))\\
	&\leq V_{t_{i}}(x^{R_{i}}_{t_{i}})-V_{t_{i}}(z^{\ast}(t_{i}))\\
	&+\left(1-\frac{t_{i+1}}{t_{i}}\right)\left(V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))\right)\\
	&+(1-\frac{t_{i+1}}{t_{i}})(g(z^{\ast}(t_{i+1}))-g(x^{0}_{t_{i+1}})).
\end{align*}
Moreover,
$$
g(x^0_{t_{i+1}})-g(z^{\ast}(t_{i+1}))\leq g(x^0_{t_{i+1}})-\Opt\leq \eta_i+\theta_{i}+\frac{2\nu}{t_i}.
$$
Since $t_{i+1}>t_{i}$, the above two inequalities imply
\begin{align*}
\frac{t_{i+1}}{t_{i}}[V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))]\leq V_{t_{i}}(x^{R_{i}}_{t_{i}})-V_{t_{i}}(z^{\ast}(t_{i}))+\frac{t_{i+1}-{t_i}}{t_{i}}(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}).
\end{align*}
Whence, 
\begin{align*}
	t_{i+1}(\Delta_{t_{i+1}}(x^{0}_{t_{i+1}}) - \theta_{i+1}) & \leq t_{i}\Delta_{t_{i}}(x^{R_{i}}_{t_{i}})+(t_{i+1}-t_{i})(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) - t_{i+1} \theta_{i+1} \\
	& \leq t_{i}(\eta_{i}+\theta_{i}) +(t_{i+1}-t_{i})(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) - t_{i+1} \theta_{i+1} \\
	& = 4 \nu + (t_{i+1}-t_{i})\cdot \frac{6\nu}{t_{i}} - 2 \nu = 2 \nu +  (1/\sigma-1)6\nu = 2\nu (3/\sigma - 2),  
	%t_{i+1}(\eta_{i}+\theta_{i})+\frac{t_{i+1}-t_{i}}{t_{i}}2\nu - t_{i+1} \theta_{i+1} = 
\end{align*}
where we used our assignments $t_{i+1}=t_i/\sigma, \eta_it_i=\theta_i t_i = 2 \nu$.
In the same way, we obtain
\begin{align*}
	\frac{\Delta_{t_{i+1}}(x^{0}_{t_{i+1}})}{\eta_{i+1}} &\leq \frac{t_{i}}{t_{i+1}\eta_{i+1}}\Delta_{t_{i}}(x^{R_{i}}_{t_{i}})+\frac{t_{i+1}-t_{i}}{t_{i+1}\eta_{i+1}}(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) \\
	&\leq \frac{t_{i}}{t_{i+1}\eta_{i+1}} (\eta_{i}+\theta_{i}) + \frac{t_{i+1}-t_{i}}{t_{i+1}\eta_{i+1}} (\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) \\
	& = \frac{4\nu }{t_{i+1}\eta_{i+1}} + \frac{t_{i+1}-t_{i}}{t_{i+1}\eta_{i+1}} \frac{6\nu}{t_{i}} = 2 + (1/\sigma-1) 3 =   (3/\sigma - 1),
\end{align*}
where we again used our assignments $t_{i+1}=t_i/\sigma, \eta_it_i=\theta_i t_i = 2 \nu$.
%In the same way, we obtain
%\begin{align*}
	%\frac{\Delta_{t_{i+1}}(x^{0}_{t_{i+1}})}{\eta_{i+1}} &\leq \frac{t_{i}}{t_{i+1}}\Delta_{t_{i}}(x^{R_{i}}_{t_{i}})+\frac{t_{i+1}-t_{i}}{t_{i+1}}(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) \\
	%&\leq \frac{t_{i}}{t_{i+1}} (\eta_{i}+\theta_{i}) + \frac{t_{i+1}-t_{i}}{t_{i+1}} (\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}) \\
	%& = \frac{2\nu }{t_{i+1}} + \frac{t_{i+1}-t_{i}}{t_{i+1}} \frac{6\nu}{t_{i}} = \frac{2\nu \sigma }{t_{i}} + (1-\sigma)  \frac{6\nu}{t_{i}} = \frac{\nu(8-6\sigma)}{t_i},
%\end{align*}
%where we again used our assignments $t_{i+1}=t_i/\sigma, \eta_it_i=\theta_i t_i = 2 \nu$.

Using these bounds, our assignments $\eta_i=\theta_i= 2 \nu/t_i$, we see that $1-10.6 t_{i} \theta_{i} <0$ and the bound \eqref{eq:IO_outer_proof_2} simplifies to
\begin{align}
\label{eq:IO_outer_proof_3}
\tilde{R}_{t_i}(x^{0}_{t_{i}},\eta_{i},\delta,\theta_{i})&\leq \left\lceil \frac{5.3(2\delta\nu (3/\sigma - 2)+\nu+t_{i}\Omega_{g})}{\delta}\log (3/\sigma - 1) \right\rceil + \left\lceil \frac{18(\nu+t_{i}\Omega_{g})^{2}}{\nu\delta^{2}}\right\rceil+1 \\
& \leq 3 + \frac{5.3(2\delta\nu (3/\sigma - 2)+\nu)}{\delta}\log (3/\sigma - 1) + \frac{18\nu}{\delta^2}\\
& \hspace{1em} + t_i \cdot \left(\frac{5.3  \Omega_{g}}{\delta}\log (3/\sigma - 1) + \frac{18 \Omega_{g}}{\delta^2} \right) + t_i^2 \cdot \frac{18 \Omega_{g}^2}{\nu\delta^2}.
\end{align}
Using the same bounds for $\sum_i t_i$, $\sum_i t_i^2$ as in the proof of \ref{th:Complexity} (see Section \ref{sec:outer}), we obtain that
\begin{align}
	\sum_{i=1}^{I}\tilde{R}_{i}&\leq \left(3 + \frac{5.3(2\delta\nu (3/\sigma - 2)+\nu)}{\delta}\log (3/\sigma - 1) + \frac{18\nu}{\delta^2} \right) \frac{\log(2\eta_{0}/\eps)}{\log(1/\sigma)} \notag  \\
	& \hspace{1em}+ \left(\frac{5.3  \Omega_{g}}{\delta}\log (3/\sigma - 1) + \frac{18 \Omega_{g}}{\delta^2} \right) \frac{4\nu}{\eps(1-\sigma)} \notag \\
	& \hspace{1em} + \frac{288 \nu \Omega_{g}^2}{\delta^2 \eps^2 (1-\sigma^2)}. \label{eq:IO_outer_proof_4}
\end{align}
Finally, we estimate $\tilde{R}_0$ as follows using \eqref{eq:IO_outer_proof_2} and that $t_0\eta_0=2\nu$, $t_0=\nu/\Omega_g$, $\theta_0=\eta_0$, $\delta <1$:
\begin{align*}
%\label{eq:IO_outer_proof_5}
\tilde{R}_0 &\leq \left\lceil \frac{5.3(t_{0}\delta\Delta_{t_{0}}(x^{0})+\nu+t_{0}\Omega_{g})}{\delta}\log\left( \frac{\Delta_{t_{0}}(x^{0})}{\eta_{0}}\right)    \right\rceil + \left\lceil \frac{18(\nu+t_{0}\Omega_{g})^{2}}{\nu\delta^{2}} \right\rceil+1\\
& \leq \frac{5.3(F(x^{0})-F(z^*(t_0))+3\nu)}{\delta}\log\left( \frac{  F(x^{0})-F(z^*(t_0))  + \nu}{2 \nu} \right)   +   \frac{72\nu}{\delta^{2}} +3.
\end{align*}
%$$
%\frac{\Delta_{t_{0}}(x^{0})}{\eta_{0}}  = \frac{ t_0^{-1} (F(x^{0})-F(z^*(t_0))) + g(x^{0})-g(z^*(t_0))}{\eta_{0}} \leq \frac{  F(x^{0})-F(z^*(t_0))  + t_0 \Omega_g}{t_0\eta_{0}} = \frac{  F(x^{0})-F(z^*(t_0))  + \nu}{2 \nu} 
%$$
Combining the latter with \eqref{eq:IO_outer_proof_4}, we obtain that the leading complexity term is $O\left( \frac{\nu \Omega_{g}^2}{\delta^2 \eps^2 (1-\sigma^2)}\right).$

We remark that assuming that the oracle accuracies $\theta_i$ have geometric decay is crucial in order to obtain the same dependence on the accuracy in the complexity as in the exact case. Indeed, if the oracle accuracy is fixed to be $\theta_i\equiv\theta$, then the last term in the bound \eqref{eq:IO_outer_proof_2} contains a term $\frac{12t_i^2\Omega_g^2\theta}{2\nu\delta^2\eta_i} = \frac{12t_i^3\Omega_g^2\theta}{4\nu^2\delta^2}$, which after summation will imply that the leading term in the complexity would be $O(1/\eps^4)$.

%==========================Analysis before 01/09/23

%\subsection{Analysis of the outer loop}
%We set $\hat{x}_{i}\equiv x^{\tilde{R}_{i}}_{t_{i}}$ the last iterate of procedure $\ICG(x^{0}_{t_{i}},t_{i},\eta_{i},\delta,\theta_{i})$, where $\tilde{R}_{i}$ is at most $R_{\tilde{G},t_{i}}(x^{0}_{t_{i}},\eta_{i},\delta,\theta_{i})$. Therefore, we know that $\widetilde{\gap}_{t_{i}}(\hat{x}_{i})\leq\eta_{i}\delta$, and a-fortiori 
%$$
%\Delta_{t_{i}}(\hat{x}_{i})\leq \gap_{t_{i}}(\hat{x}_{i})\leq \eta_{i}+\theta_{i}.  
%$$
%By eq. \ref{eq:objectivehomotopy} and the definition of the $(\delta,\theta_{i})$-\ac{ILMO}, we obtain 
%\begin{align*}
%g(\hat{x}_{i})-g(z^{\ast}(t_{i}))&\leq\gap_{t_{i}}(\hat{x}_{i})+\frac{1}{t}F'(\hat{x}_{i})[z^{\ast}(t_{i})-\hat{x}_{i}]\\
%&\leq \frac{\widetilde{\gap}_{t_{i}}(\hat{x}_{i})}{\delta}+\theta_{i}+\frac{\nu}{t_{i}}\\
%&\leq \eta_{i}+\theta_{i}+\frac{\nu}{t_{i}}.
%\end{align*}
%Hence, using \ref{lem:pathfollowing}, we observe
%$$
%g(\hat{x}_{i})-\Opt=g(\hat{x}_{i})-g(z^{\ast}(t_{i}))+g(z^{\ast}(t_{i}))-\Opt\leq \eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}.
%$$
%Since $t_{i}=\frac{2\nu}{\eta_{i}}$, we obtain $g(\hat{x}_{i})-\Opt\leq  2\eta_{i}$. We next estimate the initial gap $\Delta_{t_{i+1}}(x^{0}_{t_{i+1}})=\Delta_{t_{i+1}}(\hat{x}_{i})$ incurred by our warm-start strategy under the \ac{ILMO}. Observe that
%
%\begin{align*}
	%V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))&=V_{t_{i}}(x^{0}_{t_{i+1}})-V_{t_{i}}(z^{\ast}(t_{i+1}))\\
	%&+\left(\frac{1}{t_{i+1}}-\frac{1}{t_{i}}\right)(F(x^{0}_{t_{i+1}})-F(z^{\ast}(t_{i+1})))\\
	%&\leq V_{t_{i}}(x^{R_{i}}_{t_{i}})-V_{t_{i}}(z^{\ast}(t_{i}))\\
	%&+\left(1-\frac{t_{i+1}}{t_{i}}\right)\left(V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))\right)\\
	%&+(1-\frac{t_{i+1}}{t_{i}})(g(z^{\ast}(t_{i+1}))-g(x^{0}_{t_{i+1}})).
%\end{align*}
%
%Moreover,
%$$
%g(x^0_{t_{i+1}})-g(z^{\ast}(t_{i+1}))\leq g(x^0_{t_{i+1}})-\Opt\leq \eta_i+\theta_{i}+\frac{2\nu}{t_i}.
%$$
%Since $t_{i+1}>t_{i}$, the above two inequalities imply
%\begin{align*}
%\frac{t_{i+1}}{t_{i}}[V_{t_{i+1}}(x^{0}_{t_{i+1}})-V_{t_{i+1}}(z^{\ast}(t_{i+1}))]\leq V_{t_{i}}(x^{R_{i}}_{t_{i}})-V_{t_{i}}(z^{\ast}(t_{i}))+\frac{t_{i+1}-{t_i}}{t_{i}}(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}}).
%\end{align*}
%Whence, 
%\begin{align*}
	%t_{i+1}\Delta_{t_{i+1}}(x^{0}_{t_{i+1}})& \leq t_{i}\Delta_{t_{i}}(x^{R_{i}}_{t_{i}})+(t_{i+1}-t_{i})(\eta_{i}+\theta_{i}+\frac{2\nu}{t_{i}})\\
	%&\leq t_{i+1}(\eta_{i}+\theta_{i})+\frac{t_{i+1}-t_{i}}{t_{i}}2\nu
%\end{align*}


